A Theoretical Overview of Neural Contraction Metrics for Learning-based Control with Guaranteed Stability

This paper presents a theoretical overview of a Neural Contraction Metric (NCM): a neural network model of an optimal contraction metric and corresponding differential Lyapunov function, the existence of which is a necessary and sufficient condition for incremental exponential stability of non-autonomous nonlinear system trajectories. Its innovation lies in providing formal robustness guarantees for learning-based control frameworks, utilizing contraction theory as an analytical tool to study the nonlinear stability of learned systems via convex optimization. In particular, we rigorously show in this paper that, by regarding modeling errors of the learning schemes as external disturbances, the NCM control is capable of obtaining an explicit bound on the distance between a time-varying target trajectory and perturbed solution trajectories, which exponentially decreases with time even under the presence of deterministic and stochastic perturbation. These useful features permit simultaneous synthesis of a contraction metric and associated control law by a neural network, thereby enabling real-time computable and probably robust learning-based control for general control-affine nonlinear systems.

==> sections/note.tex <==
\textcolor{red}{focus on ``theoretical overview'' rather than ``tutorial overview''; clearly state that the objective of this paper is to provide theoretical guarantee for learning-based control using contraction theory; for example, $\|u-u_L\| \leq \epsilon_{\ell}$ in Theorem~1 should be emphasized} \textcolor{red}{talk about convexity in abstract}

==> sections/optimal_lagrange.tex <==
It is known that the following control law guarantees exponential boundedness of the system trajectories:
\begin{align}
\label{lag_con}
u &= u_n = \mathcal{H}(q)\ddot{q}_r+\mathcal{C}(q,\dot{q})\dot{q}_r+\mathcal{G}(q)-\mathcal{K}(t)s
\end{align}
where $\dot{q}_r = \dot{q}_d-\Lambda (q-q_d)$ and $s=\dot{q}-\dot{q}_r$, and that this fact can be proven by a Lyapunov function $V=s^{\top}\mathcal{H}(q)s$~\cite{Slotine:1228283}~\cite{Slotine:1228283}.

\begin{theorem}
\label{lag_clf_thm}
Suppose $\exists K: \mathbb{R}_{\leq 0}\mapsto \mathbb{R}^{n\times n}$, $\Lambda \in \mathbb{R}^n$, $\varepsilon > 0$ \st{}
\begin{align}
\begin{bmatrix} 2\mathcal{K}(t) & -\varepsilon I \\ -\varepsilon I  & 2\Lambda \end{bmatrix} \succeq 2\alpha \begin{bmatrix} \mathcal{H}(q) & 0 \\ 0 & \varepsilon I \end{bmatrix}.
\end{align}
Suppose also that \ref{sto_lag_system} is controlled by
\begin{align}
\|x-x_d\| \leq (\lambda_{\min}\left(\begin{bmatrix}I & \Lambda \\ \Lambda & I+\Lambda^2\end{bmatrix}\right))^{-\frac{1}{2}}(R(0)e^{-\alpha t}+\frac{\overline{d}}{\alpha}\frac{1}{\underline{m}})=R_{\rm NCM}(t)
\end{align}
Let $u = u_n+K^*(x,x_d,t)s = \mathcal{H}(q)\ddot{q}_r^*+\mathcal{C}(q,\dot{q})\dot{q}_r^*+\mathcal{G}(q)+K^*(x,x_d,t)s$.
\begin{align}
\label{lagrange_robust_control}
&K^*,\Lambda^* = \text{arg}\min_{K,\Lambda\in \mathbb{R}^{n\times n}}\|u-u_d\|^2 \\
\label{stability_clf}
&\text{\st{} }
\begin{bmatrix} -2K & -\varepsilon I \\ -\varepsilon I  & 2\Lambda \end{bmatrix} \succeq 2\alpha \begin{bmatrix} \mathcal{H}(q) & 0 \\ 0 & \varepsilon I \end{bmatrix}
\end{align}
\end{theorem}
